exLong: Generating Exceptional Behavior Tests with Large Language Models

Many popular programming languages, including C#, Java, and Python, support exceptions. Exceptions are thrown during program execution if an unwanted event happens, e.g., a method is invoked with an illegal argument value. Software developers write exceptional behavior tests (EBTs) to check that their code detects unwanted events and throws appropriate exceptions. Prior research studies have shown the importance of EBTs, but those studies also highlighted that developers put most of their efforts on "happy paths", e.g., paths without unwanted events. To help developers fill the gap, we present the first framework, dubbed exLong, that automatically generates EBTs. exLong is a large language model instruction fine-tuned from CodeLlama and embeds reasoning about traces that lead to throw statements, conditional expressions that guard throw statements, and non-exceptional behavior tests that execute similar traces. We compare exLong with the state-of-the-art models for test generation (CAT-LM) and one of the strongest foundation models (GPT-4o), as well as with analysis-based tools for test generation (Randoop and EvoSuite). Our results show that exLong outperforms existing models and tools. Furthermore, we contributed several pull requests to open-source projects and 23 EBTs generated by exLong were already accepted.

==> figs/collect-nodes-algorithm.tex <==
\begin{algorithm*}
\caption{Collect AST nodes along the \stacktrace (full version).}
\label{algo:node-parsing}
\small
\begin{algorithmic}[1]
\State \textbf{inputs:} \aStackTrace\ - the \stacktrace for a \ts
\State \textbf{outputs:} \aNodes\ - the collected nodes
\Procedure{\algoCollectNodes}{\aStackTrace}
\State \aNodes $\gets \emptyset$
\For{(\aMethod, $\mathtt{lineno}$) $\in$ Reversed(\aStackTrace)}
  \State $\aParsed \gets \emptyset$
  \State \aCurrent $\gets$ \textsc{GetSourceCode}(\aMethod, $\mathtt{lineno}$)
  \State $\aParent \gets \aCurrent$
  \State \aNodes $\gets$ \aNodes $\cup$ \{\aCurrent{}\}
  \While{$\aCurrent \neq \aMethod$}
    \State \aParsed $\gets$ \aParsed $\cup$ \{\aParent\}

    \If{$\aParent$ is ForStmt}
    \State \aNodes $\gets$ \aNodes $\cup$ \{\aParent.CompareExpression\}
    \EndIf

    \If{$\aParent$ is WhileStmt}
    \State \aNodes $\gets$ \aNodes $\cup$ \{\aParent.ConditionExpression\}
    \EndIf

    \If{$\aParent$ is IfStmt}
    \If{\aParent.ThenStmt == \aCurrent}
    \State \aNodes $\gets$ \aNodes $\cup$ \{\aParent.ConditionExpression\}
    \EndIf
    \If{\aParent.ElseStmt == \aCurrent}
    \State \aNodes $\gets$ \aNodes $\cup$ \{$\lnot$ \aParent.ConditionExpression\}
    \EndIf
    \EndIf

    \If{$\aParent$ is SwitchStmt}
    \State $\mathtt{selector} \gets$ \aParent.selector
    \If{$\aCurrent$ is SwitchEntry}
    \State $\mathtt{label} \gets$ \aCurrent.entryLabel
    \State $\mathtt{exp} \gets$ BinaryExpr(selector, label, EQ)
    \State \aNodes $\gets$ \aNodes $\cup$ $\{\mathtt{exp}\}$
    \Else
    \For{$\mathtt{entry} \in$ \aParent.switchEntry}
    \State $\mathtt{label} \gets$ entry.entryLabel
    \State $\mathtt{exp} \gets$ BinaryExpr(selector, label, NOT\_EQ)
    \State \aNodes $\gets$ \aNodes $\cup$ $\{\mathtt{exp}\}$
    \EndFor
    \EndIf
    \EndIf

    \If{$\aParent$ is BlockStmt}
    \For{$\mathtt{stmt}$ in \aParent.statements}
    \If{$\mathtt{stmt} \in \aParsed$}
    \State break
    \EndIf
    \If{$\mathtt{stmt}$.getExpression() is AssignExpr}
    \State \aNodes $\gets$ \aNodes $\cup$ \{$\mathtt{stmt}$.getExpression()\}
    \EndIf
    \EndFor
    \EndIf

    \State $\aCurrent = \aParent$
    \State $\aParent = \aParent$.getParent()
  \EndWhile
\EndFor
\State \Return \aNodes
\EndProcedure
\end{algorithmic}

\end{algorithm*}


==> figs/collect-nodes-cut-algorithm.tex <==
\begin{algorithm}
\caption{Collect AST nodes along the \stacktrace.}\label{algo:collect-nodes-cut}
\small
\begin{algorithmic}[1]
\State \textbf{inputs:} \aStackTrace\ - the \stacktrace for a \ts
\State \textbf{outputs:} \aNodes\ - the collected nodes
\Procedure{\algoCollectNodes}{\aStackTrace}\label{line:collect-nodes:collect-nodes}
\State \aNodes $\gets \emptyset$
\For{(\aMethod, $\mathtt{lineno}$) $\in$ Reversed(\aStackTrace)}\label{line:collect-nodes:method-loop}
\State \aCurrent $\gets$ \textsc{GetSourceCode}(\aMethod, $\mathtt{lineno}$)
% \State \aNodes $\gets$ \aNodes $\cup$ \textsc{\algoCollectNodesVisit}(\aMethod, \aStmt)
% \EndFor
% \State \Return \aNodes
% \EndProcedure
% \\
% \item[\textbf{Global var:}]\nodelist: a list containing all the interested nodes
% \item[\textbf{Inputs:}] \mn: method declaration node, \sn: the statement node to start parsing
% \item[\textbf{Outputs:}] 
% \Procedure{\algoCollectNodesVisit}{\aMethod, \aNode}\label{line:collect-nodes:visit}
% \State $\aCurrent \gets \aNode$
\State $\aParent \gets \aCurrent$
\State \aNodes $\gets$ \aNodes $\cup$ \{\aCurrent{}\} \label{line:collect-nodes:add-start-node}
\While{$\aCurrent \neq \aMethod$}
\If{$\aParent$ is ForStmt}\label{line:collect-nodes:for-beg}
\State \aNodes $\gets$ \aNodes $\cup$ \{\aParent.CompareExpression\}\label{line:collect-nodes:for-end}
\EndIf
\If{$\aParent$ is IfStmt}\label{line:collect-nodes:if-beg}
\If{\aParent.ThenStmt == \aCurrent}
\State \aNodes $\gets$ \aNodes $\cup$ \{\aParent.ConditionExpression\}
\EndIf
\If{\aParent.ElseStmt == \aCurrent}
\State \aNodes $\gets$ \aNodes $\cup$ \{$\lnot$ \aParent.ConditionExpression\}\label{line:collect-nodes:if-end}
\EndIf
\EndIf

\State \AlgoComment{Other cases (while, switch, block and assignment statements) are in supplementary material.}

\State $\aCurrent = \aParent$
\State $\aParent = \aParent$.getParent()
\EndWhile
% \EndProcedure

\EndFor
\State \Return \aNodes
\EndProcedure

\end{algorithmic}

\end{algorithm}


==> figs/compute-guardexp-algorithm.tex <==
\begin{algorithm}
\caption{Compute \guardexp based on \stacktrace.} \label{algo:compute-guardexp}
\small
\begin{algorithmic}[1]
\State \textbf{inputs:} \aStackTrace\ - the \stacktrace for a \ts
\State \textbf{outputs:} \aGuardExp\ - the \guardexp for the \ts
\Procedure{ComputeGuardExp}{\aStackTrace}
\State \aNodes $\gets$ \textsc{CollectNodes}(\aStackTrace)\label{line:compute-guardexp:collect-nodes}
\State \AlgoComment{collect all condition (if, while, etc.) and assignment (assign, method call) nodes along the \stacktrace}
\State $\aCondSet \gets \emptyset$  \AlgoComment{the set of conditions in the \guardexp}
\For{\aNode $\in$ \aNodes}\label{line:compute-guardexp:compute-beg}
\If{\aNode is ConditionalExpr}
\State \aCondSet $\gets$ \aCondSet $\cup$ \{\aNode{}\}\label{line:compute-guardexp:condition}
\EndIf
\If{\aNode is AssignStmt}
% \State $\exprmap \gets emptyMap()$
% \State $\exprmap.put(node.left, node.right)$
\State \aCondSet $\gets$ \textsc{Merge}(\aCondSet, \{\aNode.lhs $\mapsto$ \aNode.rhs\})\label{line:compute-guardexp:assignstmt}
\EndIf
\If{\aNode is MethodDeclaration}
\State $\aNode' \gets \aNode$ \AlgoComment{process with next node (method call)}
\EndIf
\If{\aNode is MethodCallExpr}
\State \aArgMap $\gets \emptyset$\label{line:method-map-0}\label{line:compute-guardexp:methodcall-beg}
\For{$\mathtt{arg}, \mathtt{argname} \in$ \aNode.getArgs(), $\aNode'$.getParams()}
\State \aArgMap $\gets$ \aArgMap $\cup \{\mathtt{argname} \mapsto \mathtt{arg}\}$
\EndFor
\State \aCondSet $\gets$ \textsc{Merge}(\aCondSet, \aArgMap)\label{line:compute-guardexp:methodcall-end}
\EndIf
\EndFor
\State \Return $\lAnd{}\aCondSet$\label{line:compute-guardexp:compute-end}
\EndProcedure
\\
\Procedure{Merge}{\aCondSet, \aArgMap}\label{line:compute-guardexp:merge}
\State \aCondSet' $\gets \emptyset$
\For{\aCond $\in$ \aCondSet}
\For{$\mathtt{name} \mapsto \mathtt{expr} \in \aArgMap$}
\If{\aCond.contains($\mathtt{name}$)}
\State \aCond $\gets$ \aCond.replace($\mathtt{name}$, $\mathtt{expr}$) \label{line:replace}
\EndIf
\EndFor
\State \aCondSet' $\gets$ \aCondSet' $\cup$ \{\aCond{}\}
\EndFor
\State \Return \aCondSet'
\EndProcedure
\end{algorithmic}
\vspace{-1pt}
\end{algorithm}



==> figs/eval-data-algorithm.tex <==
\begin{algorithm}
\caption{Prepare the pool \stacktraces from \nEBTs and assemble the prompt for evaluating \Tool.  \label{algo:eval-data}}
\small
\begin{algorithmic}[1]

\State \textbf{inputs:} \aNETestSet\ - existing \nEBTs\label{line:eval-data:input}
\State \qquad\quad\ \aSUT\ - the system under test
\State \textbf{outputs:} \aStackTraceTupleSet\ - \stacktraces to reach \tss

% % method 1: collect all stack traces
\Procedure{\algoCollectStackTraceCorpus}{\aNETestSet, \aSUT}\label{line:eval-data:stacktrace-corpus-beg}
    \State \aSUT $\gets$ InstrumentPrintTrace(\aSUT)\label{line:eval-data:instrument}
    \State \aStackTraceTupleSet $\gets \emptyset$

    \For{\aNETest $\in$ \aNETestSet}\label{line:eval-data:nebt-beg}
        \For{\aStackTrace $\in$ Execute(\aNETest)}
            % When executing one \aNETest, it is possible to get multiple \aStackTraces, because one \aNETest may invoke multiple methods.
            \State \aStackTrace $\gets$ ExcludeTestAndUtilMethods(\aStackTrace, GetFile(\aNETest))
            %% \State \aTargetMethod $\gets$ \aStackTrace{}[0].method
            \For{\aThrowStmtTarget $\in$ GetThrowStmts(\aStackTrace)}
                \State \aStackTraceTupleSet $\gets$ \aStackTraceTupleSet $\cup$ (\aStackTrace, \aNETest, \aThrowStmtTarget)\label{line:eval-data:nebt-end}
            \EndFor
        \EndFor
    \EndFor
    \State \Return \aStackTraceTupleSet
\EndProcedure\label{line:eval-data:stacktrace-corpus-end}
% % % method 2: given MUT as input, find matched stack traces
% \Procedure{FindMatchedStackTraces}{\{\aStackTrace{}\}, \aMUT}
%     \State  $\gets$ $\emptyset$
%     \For{\aStackTrace{} $\in$ \{\aStackTrace{}\}}
%         \State $ST_{mtd} = \emptyset$
%         \For{$m$ in $mtds$}
%             \If{$m \in ST$}
%                 \State $ST_{mtd} = ST_{mtd} \cup \{m\}$
%             \EndIf
%         \EndFor
%         \State $Res = Res \cup \{ST_{mtd}\}$
%     \EndFor
% \EndProcedure
\\
\State \textbf{global var:} \aStackTraceTupleSet = \textsc{\algoCollectStackTraceCorpus}(\aNETestSet, \aSUT)
\State \textbf{inputs:} \aMUT, \aThrowStmtTarget, \aTestFile\ - task inputs selected by developers or inferred\label{sec:eval-data:assemble-prompt-inputs}
\State \qquad\quad\ \aNETestSet\ - existing \nEBTs
\State \textbf{outputs:} \aPrompt\ - the prompt to give to the LLM
\Procedure{\algoAssemblePrompt}{\aMUT, \aThrowStmtTarget, \aTestFile}
\State $\mathtt{R} \gets \emptyset$
\State \aNETestSetRel $\gets \emptyset$
\For{\aStackTraceTuple $\in$ \aStackTraceTupleSet}
    \If{\aMUT $\in$ \aStackTraceTuple.\aStackTrace $\land$ \aStackTraceTuple.\aThrowStmt == \aThrowStmtTarget}\label{sec:eval-data:match}
        \State $\mathtt{R} \gets \mathtt{R}\ \cup$ \{\aStackTraceTuple.\aStackTrace{}\}
        \If{\aMUT == \aStackTraceTuple.\aStackTrace{}[0].method}
            \State \aNETestSetRel $\gets$ \aNETestSetRel $\cup$ \{\aStackTraceTuple.\aNETest{}\}\label{sec:eval-data:nebt-rel-mut}
        \EndIf
    \EndIf
\EndFor
\If {$\mathtt{R} \neq \emptyset$}
    \State \aStackTrace $\gets$ RandomSelect($\mathtt{R}$)\label{sec:eval-data:random}
    \State \aGuardExp = \textsc{ExtractGuardExp}(\aStackTrace)\label{sec:eval-data:guardexp}
    % \State \aNETestSetRel = \textsc{ExtractRelevantNEBT}(\aMUT, \aTestFile)
    \State \aNETestSetRel $\gets$ \aNETestSetRel $\cup$ $\{\aNETest | \text{GetFile}(\aNETest) \text{==} d\}$\label{sec:eval-data:nebt-rel-testfile}
    \State \Return (\aMUT, \aThrowStmtTarget, \aTestFile, \aStackTrace, \aGuardExp, \aNETestSetRel)
\EndIf
\EndProcedure

\end{algorithmic}
\end{algorithm}


==> figs/four-types-exceptions.tex <==
\begin{subfigure}[b]{0.45\linewidth}
    \begin{verbatim}
    @Test
    void tryCatch() throws Exception {
        Exception caught = null;
        try { 
            /* testing code */ 
        } catch (Exception e) { 
            caught = e; 
        }
        if (caught == null)
        fail();  // fail
        else pass();  // pass
    }
    \end{verbatim}
    \caption{Pattern try/catch. \label{fig:ebt-patterns:try-catch}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.5\linewidth}
    \begin{verbatim}
        @Test(expected = Exception.class)
        void test() throws Exception {
            /* testing code */
        }
    \end{verbatim}
    \caption{Pattern expect test. \label{fig:ebt-patterns:expect-test}}
\end{subfigure}

\begin{subfigure}[b]{0.45\linewidth}
    \begin{verbatim}
        @Rule
        ExpectedException ex;
        
        @Test
        void rule() throws Exception {
        ex = ExpectedException.none();
        ex.expect(Exception.class);
        ex.expectMessage("error");
        /* testing code */
        }
    \end{verbatim}
    \caption{Pattern expect rule. \label{fig:ebt-patterns:expect-rule}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.5\linewidth}
    \begin{verbatim}
        @Test void assert() throws Exception {
        Exception ex = Assertions.assertThrows(
            Exception.class,
            ()->{/* testing code */}
        );
        assertEquals("error", ex.getMessage());
        }
    \end{verbatim}
    \caption{Pattern assert throws. \label{fig:ebt-patterns:assert-throws}}
\end{subfigure}

==> figs/training-data-algorithm.tex <==
\begin{algorithm}
\caption{Collecting training corpus. \label{algo:training-data}}
\small
\begin{algorithmic}[1]

\State \textbf{inputs:} \aETestSet, \aNETestSet\ - existing \EBTs and \nEBTs\label{line:training-data:input}
\State \qquad\quad\ \aSUT\ - the system under test
\State \textbf{outputs:} \aCorpus\ - the training corpus of \{$(\aMUT, \aThrowStmt, \aTestFile, \aStackTrace, \aGuardExp, \aNETestSetRel, \aETest)$\}

\Procedure{CollectTrainingCorpus}{\aETestSet, \aNETestSet, \aSUT}
  \State \aCorpus $\gets$ $\emptyset$
  \For{\aETest $\in$ \aETestSet}
    % \State ProcessEBT() \AlgoComment{Wrap method body of \EBT into try-catch block}
    \State \aTestFile $\gets$ GetFile(\aETest)\label{line:training-data:tf}
    \State \aStackTrace $\gets$ Execute(InstrumentPrintException(\aETest))\label{line:training-data:stacktrace}
    \State \AlgoComment{instrumenting and executing \EBT to get \stacktrace}
    \State \aStackTrace $\gets$ ExcludeTestAndUtilMethods(\aStackTrace, \aTestFile)\label{line:training-data:stacktrace-postproc}
    \State \aMUT $\gets$ \aStackTrace{[}0].method \AlgoComment{\MUT comes first in \stacktrace}\label{line:training-data:mut}
    \State \aThrowStmt $\gets$ GetSourceCode(\aStackTrace{[}-1])\label{line:training-data:ts}
    \State \AlgoComment{last \stacktrace item points to \ts}
    \State \aGuardExp $\gets$ ComputeGuardExp(\aStackTrace)
    \State \aNETestSetRel $\gets$ $\emptyset$ \AlgoComment{initialize set of relevant \nEBTs}
    \State \aCorpus $\gets$ \aCorpus $\cup$ \{(\aMUT, \aThrowStmt, \aTestFile, \aStackTrace, \aGuardExp, \aNETestSetRel, \aETest)\}
  \EndFor

  \State \aSUT $\gets$ InstrumentPrintMethod(\aSUT)\label{line:training-data:nebt-instrumentation}
  \State \AlgoComment{instrumentation for getting methods covered by \nEBTs}
  \For{\aNETest $\in$ \aNETestSet}
    \State $\aMUT'$ $\gets$ Execute(\aNETest)[0]  
    \State \AlgoComment{get \MUT directly invoked by \nEBT}
    \For{\aCorpusItem $\in$ \aCorpus}
      \If{\aCorpusItem.\aMUT == $\aMUT' \lor$ \aCorpusItem.\aTestFile == GetFile(\aNETest)}\label{line:training-data:nebt-condition}
        \State $\aCorpusItem.\aNETestSetRel \gets \aCorpusItem.\aNETestSetRel \cup \{\aNETest\}$\label{line:training-data:nebt-add}
      \EndIf
    \EndFor
  \EndFor

  \State \Return \aCorpus
\EndProcedure
\end{algorithmic}
\vspace{-2pt}
\end{algorithm}


==> tables/numbers-elong-ablation-table.tex <==
%% Automatically generated by: paper_table.py make_numbers_results

\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-bleu}{64.17}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-bleu-avg}{64.17}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-bleu-max}{64.17}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-bleu-min}{64.17}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-code-bleu}{68.60}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-code-bleu-avg}{68.60}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-code-bleu-max}{68.60}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-code-bleu-min}{68.60}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-edit-sim}{85.78}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-edit-sim-avg}{85.78}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-edit-sim-max}{85.78}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-edit-sim-min}{85.78}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-f}{81.35}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-f-avg}{81.35}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-f-max}{81.35}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-f-min}{81.35}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-p}{83.18}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-p-avg}{83.18}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-p-max}{83.18}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-p-min}{83.18}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-r}{81.44}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-r-avg}{81.44}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-r-max}{81.44}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-r-min}{81.44}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-xmatch}{19.82}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-xmatch-top1}{19.82}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-compilable-avg}{82.49}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-compilable-max}{82.49}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-compilable-min}{82.49}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-coverage-avg}{58.53}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-coverage-max}{58.53}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-coverage-min}{58.53}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-avg}{82.40}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-max}{82.40}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-min}{82.40}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-overall}{67.97}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-overall-avg}{67.97}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-overall-max}{67.97}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-overall-min}{67.97}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-timeout-avg}{0.56}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-timeout-max}{0.56}
\DefMacro{res-elong-ablation-selected-434-conditionnestack2e-with-name-ft-lora-codellama-7b-timeout-min}{0.56}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-bleu}{64.38}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-bleu-avg}{64.38}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-bleu-max}{64.38}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-bleu-min}{64.38}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-code-bleu}{69.16}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-code-bleu-avg}{69.16}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-code-bleu-max}{69.16}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-code-bleu-min}{69.16}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-edit-sim}{86.12}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-edit-sim-avg}{86.12}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-edit-sim-max}{86.12}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-edit-sim-min}{86.12}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-f}{81.38}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-f-avg}{81.38}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-f-max}{81.38}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-f-min}{81.38}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-p}{83.32}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-p-avg}{83.32}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-p-max}{83.32}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-p-min}{83.32}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-r}{81.35}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-r-avg}{81.35}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-r-max}{81.35}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-rouge-r-min}{81.35}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-xmatch}{18.20}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-xmatch-top1}{18.20}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-compilable-avg}{82.49}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-compilable-max}{82.49}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-compilable-min}{82.49}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-coverage-avg}{56.91}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-coverage-max}{56.91}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-coverage-min}{56.91}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-runnable-avg}{81.01}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-runnable-max}{81.01}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-runnable-min}{81.01}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-runnable-overall}{66.82}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-runnable-overall-avg}{66.82}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-runnable-overall-max}{66.82}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-runnable-overall-min}{66.82}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-timeout-avg}{0.56}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-timeout-max}{0.56}
\DefMacro{res-elong-ablation-selected-434-conditionne2e-with-name-ft-lora-codellama-7b-timeout-min}{0.56}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-bleu}{63.61}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-bleu-avg}{63.61}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-bleu-max}{63.61}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-bleu-min}{63.61}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-code-bleu}{68.08}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-code-bleu-avg}{68.08}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-code-bleu-max}{68.08}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-code-bleu-min}{68.08}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-edit-sim}{85.64}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-edit-sim-avg}{85.64}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-edit-sim-max}{85.64}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-edit-sim-min}{85.64}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-f}{80.54}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-f-avg}{80.54}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-f-max}{80.54}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-f-min}{80.54}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-p}{82.41}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-p-avg}{82.41}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-p-max}{82.41}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-p-min}{82.41}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-r}{80.55}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-r-avg}{80.55}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-r-max}{80.55}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-rouge-r-min}{80.55}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-xmatch}{18.43}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-xmatch-top1}{18.43}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-compilable-avg}{80.41}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-compilable-max}{80.41}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-compilable-min}{80.41}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-coverage-avg}{49.31}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-coverage-max}{49.31}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-coverage-min}{49.31}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-runnable-avg}{75.36}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-runnable-max}{75.36}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-runnable-min}{75.36}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-runnable-overall}{60.60}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-runnable-overall-avg}{60.60}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-runnable-overall-max}{60.60}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-runnable-overall-min}{60.60}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-timeout-avg}{0.57}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-timeout-max}{0.57}
\DefMacro{res-elong-ablation-selected-434-ne2e-with-name-ft-lora-codellama-7b-timeout-min}{0.57}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-bleu}{57.17}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-bleu-avg}{57.17}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-bleu-max}{57.17}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-bleu-min}{57.17}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-code-bleu}{61.79}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-code-bleu-avg}{61.79}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-code-bleu-max}{61.79}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-code-bleu-min}{61.79}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-edit-sim}{82.30}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-edit-sim-avg}{82.30}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-edit-sim-max}{82.30}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-edit-sim-min}{82.30}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-f}{75.47}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-f-avg}{75.47}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-f-max}{75.47}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-f-min}{75.47}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-p}{78.86}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-p-avg}{78.86}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-p-max}{78.86}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-p-min}{78.86}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-r}{74.31}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-r-avg}{74.31}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-r-max}{74.31}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-rouge-r-min}{74.31}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-xmatch}{13.59}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-xmatch-avg}{13.59}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-xmatch-max}{13.59}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-xmatch-min}{13.59}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-xmatch-top1}{13.59}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-compilable-avg}{62.21}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-compilable-max}{62.21}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-compilable-min}{62.21}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-coverage-avg}{37.79}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-coverage-max}{37.79}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-coverage-min}{37.79}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-runnable-avg}{77.04}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-runnable-max}{77.04}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-runnable-min}{77.04}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-runnable-overall}{47.93}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-runnable-overall-avg}{47.93}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-runnable-overall-max}{47.93}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-runnable-overall-min}{47.93}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-timeout-avg}{0.37}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-timeout-max}{0.37}
\DefMacro{res-elong-ablation-selected-434-mut2e-with-name-ft-lora-codellama-7b-timeout-min}{0.37}


==> tables/numbers-gpt4o-exlong-table.tex <==
%% Automatically generated by: paper_table.py make_numbers

\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-bleu}{60.07}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-bleu-avg}{60.07}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-bleu-max}{60.07}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-bleu-min}{60.07}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-code-bleu}{65.56}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-code-bleu-avg}{65.56}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-code-bleu-max}{65.56}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-code-bleu-min}{65.56}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-edit-sim}{84.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-edit-sim-avg}{84.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-edit-sim-max}{84.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-edit-sim-min}{84.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-f}{78.30}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-f-avg}{78.30}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-f-max}{78.30}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-f-min}{78.30}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-p}{80.36}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-p-avg}{80.36}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-p-max}{80.36}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-p-min}{80.36}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-r}{78.60}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-r-avg}{78.60}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-r-max}{78.60}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-rouge-r-min}{78.60}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-xmatch}{16.82}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-xmatch-avg}{16.82}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-xmatch-max}{16.82}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-xmatch-min}{16.82}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-xmatch-top1}{16.82}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-compilable-avg}{81.87}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-compilable-max}{81.87}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-compilable-min}{81.87}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-coverage-avg}{55.53}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-coverage-max}{55.53}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-coverage-min}{55.53}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-match-avg}{99.73}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-match-max}{99.73}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-match-min}{99.73}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-runnable-avg}{87.60}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-runnable-max}{87.60}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-runnable-min}{87.60}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-runnable-overall}{71.52}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-runnable-overall-avg}{71.52}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-runnable-overall-max}{71.52}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-runnable-overall-min}{71.52}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-timeout-avg}{0.28}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-timeout-max}{0.28}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-with-name-gpt-4o-timeout-min}{0.28}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-bleu}{60.48}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-bleu-avg}{60.48}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-bleu-max}{60.48}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-bleu-min}{60.48}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-code-bleu}{66.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-code-bleu-avg}{66.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-code-bleu-max}{66.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-code-bleu-min}{66.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-edit-sim}{84.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-edit-sim-avg}{84.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-edit-sim-max}{84.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-edit-sim-min}{84.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-f}{79.24}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-f-avg}{79.24}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-f-max}{79.24}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-f-min}{79.24}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-p}{80.33}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-p-avg}{80.33}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-p-max}{80.33}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-p-min}{80.33}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-r}{80.30}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-r-avg}{80.30}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-r-max}{80.30}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-rouge-r-min}{80.30}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-xmatch}{17.74}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-xmatch-avg}{17.74}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-xmatch-max}{17.74}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-xmatch-min}{17.74}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-xmatch-top1}{17.74}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-compilable-avg}{82.49}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-compilable-max}{82.49}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-compilable-min}{82.49}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-coverage-avg}{64.75}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-coverage-max}{64.75}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-coverage-min}{64.75}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-match-avg}{100.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-match-max}{100.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-match-min}{100.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-runnable-avg}{91.34}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-runnable-max}{91.34}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-runnable-min}{91.34}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-runnable-overall}{75.35}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-runnable-overall-avg}{75.35}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-runnable-overall-max}{75.35}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-runnable-overall-min}{75.35}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-timeout-avg}{0.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-timeout-max}{0.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-with-name-gpt-4o-timeout-min}{0.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-bleu}{40.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-bleu-avg}{40.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-bleu-max}{40.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-bleu-min}{40.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-code-bleu}{51.42}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-code-bleu-avg}{51.42}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-code-bleu-max}{51.42}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-code-bleu-min}{51.42}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-edit-sim}{69.63}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-edit-sim-avg}{69.63}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-edit-sim-max}{69.63}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-edit-sim-min}{69.63}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-f}{69.66}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-f-avg}{69.66}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-f-max}{69.66}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-f-min}{69.66}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-p}{71.08}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-p-avg}{71.08}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-p-max}{71.08}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-p-min}{71.08}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-r}{70.54}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-r-avg}{70.54}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-r-max}{70.54}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-rouge-r-min}{70.54}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-xmatch}{0.46}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-xmatch-avg}{0.46}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-xmatch-max}{0.46}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-xmatch-min}{0.46}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-xmatch-top1}{0.46}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-compilable-avg}{79.95}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-compilable-max}{79.95}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-compilable-min}{79.95}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-coverage-avg}{42.63}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-coverage-max}{42.63}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-coverage-min}{42.63}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-match-avg}{99.71}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-match-max}{99.71}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-match-min}{99.71}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-runnable-avg}{80.35}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-runnable-max}{80.35}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-runnable-min}{80.35}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-runnable-overall}{64.06}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-runnable-overall-avg}{64.06}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-runnable-overall-max}{64.06}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-runnable-overall-min}{64.06}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-timeout-avg}{0.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-timeout-max}{0.00}
\DefMacro{res-gpt4o-exlong-ne2e-few-shot-no-name-gpt-4o-timeout-min}{0.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-bleu}{43.62}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-bleu-avg}{43.62}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-bleu-max}{43.62}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-bleu-min}{43.62}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-code-bleu}{54.47}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-code-bleu-avg}{54.47}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-code-bleu-max}{54.47}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-code-bleu-min}{54.47}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-edit-sim}{74.11}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-edit-sim-avg}{74.11}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-edit-sim-max}{74.11}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-edit-sim-min}{74.11}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-f}{71.93}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-f-avg}{71.93}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-f-max}{71.93}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-f-min}{71.93}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-p}{73.09}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-p-avg}{73.09}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-p-max}{73.09}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-p-min}{73.09}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-r}{72.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-r-avg}{72.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-r-max}{72.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-rouge-r-min}{72.77}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-xmatch}{0.69}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-xmatch-avg}{0.69}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-xmatch-max}{0.69}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-xmatch-min}{0.69}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-xmatch-top1}{0.69}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-compilable-avg}{80.88}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-compilable-max}{80.88}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-compilable-min}{80.88}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-coverage-avg}{62.67}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-coverage-max}{62.67}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-coverage-min}{62.67}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-match-avg}{100.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-match-max}{100.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-match-min}{100.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-runnable-avg}{89.74}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-runnable-max}{89.74}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-runnable-min}{89.74}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-runnable-overall}{72.58}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-runnable-overall-avg}{72.58}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-runnable-overall-max}{72.58}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-runnable-overall-min}{72.58}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-timeout-avg}{0.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-timeout-max}{0.00}
\DefMacro{res-gpt4o-exlong-conditionnestack2e-few-shot-no-name-gpt-4o-timeout-min}{0.00}


==> tables/numbers-models-results.tex <==
%% Automatically generated by: Table.py make_numbers_results

\DefMacro{res-mut2e-zero-shot-gpt-4-0613-bleu}{47.40}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-bleu-avg}{47.40}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-bleu-max}{47.40}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-bleu-min}{47.40}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-code-bleu}{53.59}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-code-bleu-avg}{53.59}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-code-bleu-max}{53.59}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-code-bleu-min}{53.59}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-edit-sim}{76.54}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-edit-sim-avg}{76.54}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-edit-sim-max}{76.54}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-edit-sim-min}{76.54}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-f}{67.95}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-f-avg}{67.95}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-f-max}{67.95}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-f-min}{67.95}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-p}{69.15}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-p-avg}{69.15}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-p-max}{69.15}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-p-min}{69.15}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-r}{69.35}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-r-avg}{69.35}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-r-max}{69.35}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-rouge-r-min}{69.35}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-xmatch}{7.96}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-xmatch-top1}{7.96}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-compilable-avg}{66.86}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-compilable-max}{66.86}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-compilable-min}{66.86}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-match-avg}{99.47}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-match-max}{99.47}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-match-min}{99.47}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-runnable-avg}{82.39}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-runnable-max}{82.39}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-runnable-min}{82.39}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-timeout-avg}{0.18}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-timeout-max}{0.18}
\DefMacro{res-mut2e-zero-shot-gpt-4-0613-timeout-min}{0.18}
\DefMacro{res-mut2e-zero-shot-gpt3.5-bleu}{43.44}
\DefMacro{res-mut2e-zero-shot-gpt3.5-bleu-avg}{43.44}
\DefMacro{res-mut2e-zero-shot-gpt3.5-bleu-max}{43.44}
\DefMacro{res-mut2e-zero-shot-gpt3.5-bleu-min}{43.44}
\DefMacro{res-mut2e-zero-shot-gpt3.5-code-bleu}{51.07}
\DefMacro{res-mut2e-zero-shot-gpt3.5-code-bleu-avg}{51.07}
\DefMacro{res-mut2e-zero-shot-gpt3.5-code-bleu-max}{51.07}
\DefMacro{res-mut2e-zero-shot-gpt3.5-code-bleu-min}{51.07}
\DefMacro{res-mut2e-zero-shot-gpt3.5-edit-sim}{74.08}
\DefMacro{res-mut2e-zero-shot-gpt3.5-edit-sim-avg}{74.08}
\DefMacro{res-mut2e-zero-shot-gpt3.5-edit-sim-max}{74.08}
\DefMacro{res-mut2e-zero-shot-gpt3.5-edit-sim-min}{74.08}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-f}{65.26}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-f-avg}{65.26}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-f-max}{65.26}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-f-min}{65.26}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-p}{63.51}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-p-avg}{63.51}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-p-max}{63.51}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-p-min}{63.51}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-r}{70.98}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-r-avg}{70.98}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-r-max}{70.98}
\DefMacro{res-mut2e-zero-shot-gpt3.5-rouge-r-min}{70.98}
\DefMacro{res-mut2e-zero-shot-gpt3.5-xmatch}{5.97}
\DefMacro{res-mut2e-zero-shot-gpt3.5-xmatch-top1}{5.97}
\DefMacro{res-mut2e-zero-shot-gpt3.5-compilable-avg}{54.57}
\DefMacro{res-mut2e-zero-shot-gpt3.5-compilable-max}{54.57}
\DefMacro{res-mut2e-zero-shot-gpt3.5-compilable-min}{54.57}
\DefMacro{res-mut2e-zero-shot-gpt3.5-match-avg}{100.00}
\DefMacro{res-mut2e-zero-shot-gpt3.5-match-max}{100.00}
\DefMacro{res-mut2e-zero-shot-gpt3.5-match-min}{100.00}
\DefMacro{res-mut2e-zero-shot-gpt3.5-runnable-avg}{78.54}
\DefMacro{res-mut2e-zero-shot-gpt3.5-runnable-max}{78.54}
\DefMacro{res-mut2e-zero-shot-gpt3.5-runnable-min}{78.54}
\DefMacro{res-mut2e-zero-shot-gpt3.5-timeout-avg}{0.00}
\DefMacro{res-mut2e-zero-shot-gpt3.5-timeout-max}{0.00}
\DefMacro{res-mut2e-zero-shot-gpt3.5-timeout-min}{0.00}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-bleu}{57.17}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-bleu-avg}{57.17}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-bleu-max}{57.17}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-bleu-min}{57.17}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-code-bleu}{61.62}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-code-bleu-avg}{61.62}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-code-bleu-max}{61.62}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-code-bleu-min}{61.62}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-edit-sim}{82.64}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-edit-sim-avg}{82.64}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-edit-sim-max}{82.64}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-edit-sim-min}{82.64}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-f}{74.75}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-f-avg}{74.75}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-f-max}{74.75}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-f-min}{74.75}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-p}{77.17}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-p-avg}{77.17}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-p-max}{77.17}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-p-min}{77.17}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-r}{74.68}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-r-avg}{74.68}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-r-max}{74.68}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-rouge-r-min}{74.68}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-xmatch}{9.62}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-xmatch-top1}{9.62}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-compilable-avg}{62.95}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-compilable-max}{62.95}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-compilable-min}{62.95}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-runnable-avg}{82.08}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-runnable-max}{82.08}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-runnable-min}{82.08}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-runnable-overall}{51.66}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-timeout-avg}{0.38}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-timeout-max}{0.38}
\DefMacro{res-mut2e-with-name-ft-lora-codellama-7b-timeout-min}{0.38}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-bleu}{38.08}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-bleu-avg}{38.08}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-bleu-max}{38.08}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-bleu-min}{38.08}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-code-bleu}{46.34}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-code-bleu-avg}{46.34}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-code-bleu-max}{46.34}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-code-bleu-min}{46.34}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-edit-sim}{73.02}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-edit-sim-avg}{73.02}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-edit-sim-max}{73.02}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-edit-sim-min}{73.02}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-f}{66.15}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-f-avg}{66.15}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-f-max}{66.15}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-f-min}{66.15}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-p}{68.72}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-p-avg}{68.72}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-p-max}{68.72}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-p-min}{68.72}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-r}{65.84}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-r-avg}{65.84}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-r-max}{65.84}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-rouge-r-min}{65.84}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-xmatch}{0.24}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-xmatch-top1}{0.24}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-compilable-avg}{64.85}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-compilable-max}{64.85}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-compilable-min}{64.85}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-runnable-avg}{73.63}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-runnable-max}{73.63}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-runnable-min}{73.63}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-runnable-overall}{47.74}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-timeout-avg}{0.37}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-timeout-max}{0.37}
\DefMacro{res-mut2e-no-name-ft-lora-codellama-7b-timeout-min}{0.37}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-bleu}{61.81}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-bleu-avg}{61.81}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-bleu-max}{61.81}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-bleu-min}{61.81}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-code-bleu}{66.27}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-code-bleu-avg}{66.27}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-code-bleu-max}{66.27}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-code-bleu-min}{66.27}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-edit-sim}{84.86}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-edit-sim-avg}{84.86}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-edit-sim-max}{84.86}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-edit-sim-min}{84.86}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-f}{79.03}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-f-avg}{79.03}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-f-max}{79.03}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-f-min}{79.03}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-p}{80.17}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-p-avg}{80.17}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-p-max}{80.17}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-p-min}{80.17}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-r}{80.00}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-r-avg}{80.00}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-r-max}{80.00}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-rouge-r-min}{80.00}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-xmatch}{14.61}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-xmatch-top1}{14.61}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-compilable-avg}{79.93}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-compilable-max}{79.93}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-compilable-min}{79.93}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-runnable-avg}{76.97}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-runnable-max}{76.97}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-runnable-min}{76.97}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-runnable-overall}{61.52}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-timeout-avg}{0.45}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-timeout-max}{0.45}
\DefMacro{res-ne2e-with-name-ft-lora-codellama-7b-timeout-min}{0.45}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-bleu}{43.32}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-bleu-avg}{43.32}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-bleu-max}{43.32}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-bleu-min}{43.32}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-code-bleu}{51.19}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-code-bleu-avg}{51.19}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-code-bleu-max}{51.19}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-code-bleu-min}{51.19}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-edit-sim}{77.48}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-edit-sim-avg}{77.48}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-edit-sim-max}{77.48}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-edit-sim-min}{77.48}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-f}{71.02}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-f-avg}{71.02}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-f-max}{71.02}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-f-min}{71.02}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-p}{72.97}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-p-avg}{72.97}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-p-max}{72.97}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-p-min}{72.97}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-r}{71.08}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-r-avg}{71.08}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-r-max}{71.08}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-rouge-r-min}{71.08}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-xmatch}{0.71}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-xmatch-top1}{0.71}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-compilable-avg}{83.14}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-compilable-max}{83.14}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-compilable-min}{83.14}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-runnable-avg}{75.29}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-runnable-max}{75.29}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-runnable-min}{75.29}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-runnable-overall}{62.59}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-timeout-avg}{0.29}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-timeout-max}{0.29}
\DefMacro{res-ne2e-no-name-ft-lora-codellama-7b-timeout-min}{0.29}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-bleu}{63.19}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-bleu-avg}{63.19}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-bleu-max}{63.19}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-bleu-min}{63.19}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-code-bleu}{67.34}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-code-bleu-avg}{67.34}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-code-bleu-max}{67.34}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-code-bleu-min}{67.34}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-edit-sim}{85.39}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-edit-sim-avg}{85.39}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-edit-sim-max}{85.39}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-edit-sim-min}{85.39}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-f}{80.22}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-f-avg}{80.22}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-f-max}{80.22}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-f-min}{80.22}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-p}{81.65}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-p-avg}{81.65}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-p-max}{81.65}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-p-min}{81.65}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-r}{80.73}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-r-avg}{80.73}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-r-max}{80.73}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-rouge-r-min}{80.73}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-xmatch}{14.96}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-xmatch-top1}{14.96}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-compilable-avg}{77.92}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-compilable-max}{80.76}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-compilable-min}{73.75}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-runnable-avg}{80.85}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-runnable-max}{83.24}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-runnable-min}{77.79}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-runnable-overall}{63.00}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-timeout-avg}{0.44}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-timeout-max}{0.44}
\DefMacro{res-nestack2e-with-name-ft-lora-codellama-7b-timeout-min}{0.44}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-compilable-avg}{80.17}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-compilable-max}{80.17}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-compilable-min}{80.17}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-runnable-avg}{83.26}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-runnable-max}{83.26}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-runnable-min}{83.26}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-runnable-overall}{66.75}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-timeout-avg}{0.30}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-timeout-max}{0.30}
\DefMacro{res-gt-nestack2e-with-name-ft-lora-codellama-7b-timeout-min}{0.30}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-bleu}{45.12}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-bleu-avg}{45.12}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-bleu-max}{45.12}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-bleu-min}{45.12}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-code-bleu}{53.70}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-code-bleu-avg}{53.70}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-code-bleu-max}{53.70}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-code-bleu-min}{53.70}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-edit-sim}{79.03}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-edit-sim-avg}{79.03}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-edit-sim-max}{79.03}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-edit-sim-min}{79.03}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-f}{73.07}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-f-avg}{73.07}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-f-max}{73.07}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-f-min}{73.07}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-p}{74.74}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-p-avg}{74.74}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-p-max}{74.74}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-p-min}{74.74}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-r}{73.27}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-r-avg}{73.27}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-r-max}{73.27}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-rouge-r-min}{73.27}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-xmatch}{1.31}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-xmatch-top1}{1.31}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-compilable-avg}{81.24}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-compilable-max}{81.24}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-compilable-min}{81.24}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-runnable-avg}{82.60}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-runnable-max}{82.60}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-runnable-min}{82.60}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-runnable-overall}{67.10}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-timeout-avg}{0.15}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-timeout-max}{0.15}
\DefMacro{res-nestack2e-no-name-ft-lora-codellama-7b-timeout-min}{0.15}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-bleu}{63.69}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-bleu-avg}{63.69}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-bleu-max}{63.69}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-bleu-min}{63.69}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-code-bleu}{67.49}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-code-bleu-avg}{67.49}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-code-bleu-max}{67.49}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-code-bleu-min}{67.49}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-edit-sim}{86.43}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-edit-sim-avg}{86.43}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-edit-sim-max}{86.43}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-edit-sim-min}{86.43}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-f}{80.60}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-f-avg}{80.60}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-f-max}{80.60}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-f-min}{80.60}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-p}{82.11}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-p-avg}{82.11}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-p-max}{82.11}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-p-min}{82.11}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-r}{80.82}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-r-avg}{80.82}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-r-max}{80.82}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-rouge-r-min}{80.82}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-xmatch}{14.13}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-xmatch-top1}{14.13}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-compilable-avg}{78.98}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-compilable-max}{78.98}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-compilable-min}{78.98}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-runnable-avg}{82.56}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-runnable-max}{82.56}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-runnable-min}{82.56}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-runnable-overall}{65.20}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-timeout-avg}{0.30}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-timeout-max}{0.30}
\DefMacro{res-conditionne2e-with-name-ft-lora-codellama-7b-timeout-min}{0.30}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-bleu}{45.46}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-bleu-avg}{45.46}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-bleu-max}{45.46}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-bleu-min}{45.46}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-code-bleu}{53.49}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-code-bleu-avg}{53.49}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-code-bleu-max}{53.49}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-code-bleu-min}{53.49}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-edit-sim}{79.40}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-edit-sim-avg}{79.40}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-edit-sim-max}{79.40}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-edit-sim-min}{79.40}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-f}{73.33}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-f-avg}{73.33}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-f-max}{73.33}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-f-min}{73.33}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-p}{75.07}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-p-avg}{75.07}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-p-max}{75.07}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-p-min}{75.07}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-r}{73.36}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-r-avg}{73.36}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-r-max}{73.36}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-rouge-r-min}{73.36}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-xmatch}{1.07}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-xmatch-top1}{1.07}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-compilable-avg}{81.00}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-compilable-max}{81.00}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-compilable-min}{81.00}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-runnable-avg}{80.65}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-runnable-max}{80.65}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-runnable-min}{80.65}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-runnable-overall}{65.32}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-timeout-avg}{0.00}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-timeout-max}{0.00}
\DefMacro{res-conditionne2e-no-name-ft-lora-codellama-7b-timeout-min}{0.00}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-bleu}{62.41}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-bleu-avg}{62.41}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-bleu-max}{62.41}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-bleu-min}{62.41}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-code-bleu}{66.77}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-code-bleu-avg}{66.77}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-code-bleu-max}{66.77}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-code-bleu-min}{66.77}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-edit-sim}{85.37}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-edit-sim-avg}{85.37}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-edit-sim-max}{85.37}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-edit-sim-min}{85.37}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-f}{79.95}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-f-avg}{79.95}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-f-max}{79.95}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-f-min}{79.95}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-p}{80.99}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-p-avg}{80.99}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-p-max}{80.99}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-p-min}{80.99}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-r}{80.97}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-r-avg}{80.97}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-r-max}{80.97}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-rouge-r-min}{80.97}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-xmatch}{14.61}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-xmatch-top1}{14.61}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-compilable-avg}{79.22}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-compilable-max}{79.22}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-compilable-min}{79.22}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-avg}{84.41}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-max}{84.41}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-min}{84.41}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-runnable-overall}{66.86}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-timeout-avg}{0.30}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-timeout-max}{0.30}
\DefMacro{res-conditionnestack2e-with-name-ft-lora-codellama-7b-timeout-min}{0.30}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-bleu}{45.63}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-bleu-avg}{45.63}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-bleu-max}{45.63}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-bleu-min}{45.63}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-code-bleu}{53.74}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-code-bleu-avg}{53.74}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-code-bleu-max}{53.74}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-code-bleu-min}{53.74}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-edit-sim}{79.53}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-edit-sim-avg}{79.53}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-edit-sim-max}{79.53}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-edit-sim-min}{79.53}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-f}{73.49}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-f-avg}{73.49}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-f-max}{73.49}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-f-min}{73.49}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-p}{75.53}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-p-avg}{75.53}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-p-max}{75.53}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-p-min}{75.53}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-r}{73.31}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-r-avg}{73.31}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-r-max}{73.31}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-rouge-r-min}{73.31}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-xmatch}{1.07}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-xmatch-top1}{1.07}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-compilable-avg}{81.00}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-compilable-max}{81.00}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-compilable-min}{81.00}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-match-avg}{100.00}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-match-max}{100.00}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-match-min}{100.00}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-runnable-avg}{85.92}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-runnable-max}{85.92}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-runnable-min}{85.92}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-runnable-overall}{69.60}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-timeout-avg}{0.29}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-timeout-max}{0.29}
\DefMacro{res-conditionnestack2e-no-name-ft-lora-codellama-7b-timeout-min}{0.29}

